Augment Before Copy-Paste: Data and Memory Efficiency-Oriented Instance Segmentation Framework for Sport-scenes

Instance segmentation is a fundamental task in computer vision with broad applications across various industries. In recent years, with the proliferation of deep learning and artificial intelligence applications, how to train effective models with limited data has become a pressing issue for both academia and industry. In the Visual Inductive Priors challenge (VIPriors2023), participants must train a model capable of precisely locating individuals on a basketball court, all while working with limited data and without the use of transfer learning or pre-trained models. We propose Memory effIciency inStance Segmentation framework based on visual inductive prior flow propagation that effectively incorporates inherent prior information from the dataset into both the data preprocessing and data augmentation stages, as well as the inference phase. Our team (ACVLAB) experiments demonstrate that our model achieves promising performance (0.509 AP@0.50:0.95) even under limited data and memory constraints.

==> articles/model.tex <==

%\section{Model Architecture}
%\label{sec:Model Architecture}


%Our model is architecturally founded on the HybridTaskCascade  \cite{HTC} detector. Subsequent to this foundation, we utilize the CB-SwinTransformer-Base \cite{CBNet}\cite{swin} as our backbone to extract image features. After this, we integrate the CB-feature pyramid network, which employs group normalization \cite{groupnormalization} as model's neck to better capture  from low to high-level feature representations. As for model's head parts, we use the region proposal network with its default setting. This is further followed by the inclusion of the HybridTaskCascadeRoIHead. Within this RoI head, there are two pivotal components: the bounding-bbox head, which retains its default setting, and the mask-head. The mask-head is replaced by mask-scoring head \cite{MaskScoringRCNN} to improve model performance on instance's texture and boundary details.

%\begin{figure*}
%	\centering
	%\includegraphics[width=0.9\textwidth]{image/model demo.png}
	%\caption{Overall architecture of the proposed model for VIPrior instance segmentation challenge 2023.}
	%\label{fig:flowchart.png}	
%\end{figure*}

==> articles/related.tex <==
% !TEX root = ../main.tex

\section{Related Work}
\label{sec:related}
\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{image/demo6.png}
    \caption{The overall  of proposed instance segmentation framework. The visual inductive prior is fully utilized at each stage to make effective optimizations. This approach not only reduces computational resource consumption but also maintains solid model performance}
    \label{fig:overall.png}	
\end{figure*}
\subsection{Instance Segmentation Model}
In recent years, deep learning-based instance segmentation methods have garnered widespread recognition, exemplified by approaches such as Cascade-MaskRCNN\cite{CascadeRCNN}, Maskformer\cite{Maskformer}, queryinst\cite{QueryInst}, and CBNet\cite{CBNet}, among others. Over the past couple of years, \cite{2021sota}\cite{2022sota}. have demonstrated remarkable achievements within the VIPriors Workshop through the CBNet-based model architectures.

CBNet is distinguished by its capability to synergistically couple multiple backbone networks and detectors, enabling the effective fusion of both low-level and high-level semantic representations. This architecture, characterized by its scalability and ease of training, imparts a diverse range of model inductive attributes. It accomplishes this while maintaining noteworthy detection precision and generalization ability without compromising inference speed.


\subsection{Data Augmentation}

Data augmentation constitutes a critical facet in training deep learning models, especially when confronted with limited data. By subjecting original images to operations such as hue variations, geometric transformations, and erasure transformations, the diversity of features is augmented, enhancing the model's capacity for generalization across unseen domains.

Copy-paste augmentation\cite{CopyPaste} emerges as an effective augmentation strategy for instance segmentation task. It leverages prior knowledge of objects to enhance a model's generalization and robustness to out-of-domain objects. In VIPriors instance segmentation challenge , \cite{2021sota}\cite{2022sota} introduced task-specific copy-paste augmentation. This procedure leverages object-derived visual prior knowledge to optimize the data pipeline, ensuring that the features of pasted objects align more closely with plausible scenarios.
For instance, constraints can be applied to the coordinates of pasted images based on the probable player positions, effectively filtering out implausible results.





%\subsection{Mask training}
%In the realm of Natural Language Processing, substantial success has been achieved through mask training. By replacing tokens with masks, the model's ability to understand contextual semantics can be enhanced, such as BERT\cite{BERT}. He et al. \cite{MaskedAutoencoders2021}introduced the concept of mask training into the computer vision domain. Specifically, images are encoded into multiple patches, with certain patches being masked during the encoding process. This training methodology, which disrupts the original signal, enables the decoder to glean contextual information more comprehensively. This learning paradigm has found widespread applications within the field of computer vision.
